Cross-modal Variational Auto-encoder with Distributed Latent Spaces and Associators

In this paper, we propose a novel structure for a cross-modal data association, which is inspired by the recent research on the associative learning structure of the brain. We formulate the cross-modal association in Bayesian inference framework realized by a deep neural network with multiple variational auto-encoders and variational associators. The variational associators transfer the latent spaces between auto-encoders that represent different modalities. The proposed structure successfully associates even heterogeneous modal data and easily incorporates the additional modality to the entire network via the proposed cross-modal associator. Furthermore, the proposed structure can be trained with only a small amount of paired data since auto-encoders can be trained by unsupervised manner. Through experiments, the effectiveness of the proposed structure is validated on various datasets including visual and auditory data.

==> 6-Rebuttal.tex <==

\noindent \textbf{1. Gaussian approximation for $q(\textbf{z}_j|\textbf{x}_i)$ in (9): }
As commented,  $q(\textbf{z}_j|\textbf{x}_i)$ in (9) is a Gaussian mixture. However, it is intractable to calculate KL divergence for a Gaussian mixture. Following the existing studies
$^[$\footnote{J. Hershey, et. al., ``Approximating KL divergence between gaussian mixture models," ICASSP 2007, p. IV–317.
}$^,$\footnote{M. Huber, et. al., ``On entropy approximation for gaussian mixture," MFI 2008, pp. 181–188.}$^]$, 
we approximated this as a Gaussian to obtain KL divergence.


\noindent \textbf{2. Influence of the log-ratio term in (6): }
We derived (7) under the assumption that the log-ratio term in (6) is negligible. We have conducted a new experiment by including the term. As shown in Table~\ref{tabular:cross}, the new result (\textit{ours-all}) was similar to the original result (\textit{ours}). In the final paper, we will revise the manuscript to include the log-ratio term.


\noindent \textbf{3. Comparison with recent methods: }
Three recent methods$^[$\footnote{M. Suzuki, et. al., ``Joint multimodal learning with deep generative models," ICLR workshop 2017,  
arXiv:1611.01891.}$^,$\footnote{M. Wu, et. al., ``Multimodal generative models for scalable weakly-supervised learning," NIPS 2018, 
arXiv:1802.05335.}$^]$
were compared additionally.
As shown in Table~\ref{tabular:cross}, our method outperforms these recent methods and shows a large amount of enhancement when generating voice modality (GSC) from other modality inputs.

\noindent \textbf{4. Novelty: }
A distinctive aspect of the proposed structure is the {\it associator} embedded between the auto-encoders, along with its realization designed as a variational inference framework. This associator offers many advantages in terms of flexibility, scalability, and generalizability. We believe that this advantage could contribute to meaningful progress in developing large-size multi-modal association machines, as described below.

\noindent \textbf{Flexibility. }
Our structure can provide a flexible dimensional encoding in each latent space depending on the complexity of each modality. In existing methods (CVA, JMVAE), the latent space is shared among every modality, so its dimension must be the same for every modality. As shown in Table~\ref{tabular:cross}~(\textit{ours-flex}), the enhanced performance was achieved by adopting a flexible dimension depending on the complexity of each modality.
In addition, when handling heterogeneous modalities, the shared latent space could be biased to the dominant modality. However, in our methods, the associator acts as a translator between modalities, and thus the characteristics of each latent space are preserved. Table~\ref{tabular:cross} shows that our method achieves a good performance in both directions, whereas the other methods show a degraded performance in the direction to GSC.

\input{tables/comparison_rebuttal.tex}

\noindent \textbf{Scalability. } 
Our structure can easily expand a new modality while maintaining the existing modalities. That is, a new modality can be added via training of only a new associator between an existing auto-encoder and a new auto-encoder. To validate this aspect, 
we added an additional associator between MNIST and Fashion-MNIST(F-MNIST) modalities.
As given in the following table,
the proposed model can achieve a good association between F-MNIST and GSC without a direct associator between F-MNIST and GSC.

\input{tables/scalability_rebuttal.tex}

\noindent
\textbf{Generalizability.}  
Figure 6 in Section 4.4 in the submitted manuscript depicts that our model, trained on a small portion of paired data, has not so much difference in performance from that trained with full data. This result implies that our structure with associator gives a good generalization performance even by semi-supervised learning.


\noindent \textbf{5. Details of the experiment setting: }
Since quantitative measures depend on the recognizer, it is fair to use the same recognizer for all methods for consistent evaluation.
Thus we build a recognizer from the data space rather than latent space
which varies depending on a model.
The number of paired data is $31158$ for $10$ classes of (MNIST$\rightarrow$GSC) and $3419$ for $4$ classes of (GTSRB$\rightarrow$GSC).


\noindent \textbf{6. Experiments on Hand pose.}
We have conducted additional experiments on the Hand pose dataset used in CVA. The  \textit{reconstruction errors} are given in the following Table. Even when using only the basic option (T), our model outperforms CVA using all the options (T+S+H).
\jw{여기서 $T+S+H$는 실험 불가? 또, 예전에 이 테이블이랑 CVA랑 메져가 다르다고 한 것 같은데 그부분은 일치 불가?} \jw{개인적으로 Hand Pose 쪽이 Real-world 데이터로서의 임팩트가 있어서 이 실험은 Supple이 아닌 본문에 추가하는 편이 좋을 것 같음. 가능하다면 Qualitative 결과도 추가.}

\input{tables/handpose_rebuttal.tex}

\noindent \textbf{7. Improving the manuscript:}
In the camera ready, we will incorporate all the aforementioned issues.
In addition, we will supplement the survey and discussion of related studies
and tone-down the neuroscientific motivation. 




==> 7-Note.tex <==
% \begin{itemize}
    % \item \dw{Encoding decoding을 거치면서 정교해지는 것에 대한 내용 추가, ablation test, 가능하다면 정성적 평가, recurrent, Hopfield network의 noisy surpression}
    % \item \dw{recursion 돌릴수록 변화하는 것 보기}
    % \item \dw{Flexibility에 대한 내용을 조금 수정. 분리하는 것이 합쳐놓은거보다 좋다는 것 강조.}
    % \item \dw{다른 비교실험에 대해서도 그림결과 뽑기}
    % \item \dw{용어나 흐름을 조금 더 깔끔하게 정리하기}
    % \item \dw{알고리즘의 이름을 정해서 논문안에서 부르는 것이 더 편할까? ex. CroMA}
    % \item \dw{우리 것이 이질적인 modality에대해서 잘 된다는 것을 어필하기 위해서 이질적이지 않은 것에 대한 실험도 추가하는 것}
    % \item \dw{ablation test 내용 변경, 특히 associator의 장점을 강조하는 방향으로.}
% \end{itemize}


==> figure_brain.tex <==
\begin{figure}
\centering 
\includegraphics[width=\linewidth]{figures/fig_cortex.pdf}
\caption{
\textbf{Example of how the brain memorizes multi-modal associative data}
Intra-modal associative memory cells (highlighted cells) in the visual cortex are trained to discriminate various sensory data (images of an apple, an orange and a banana) through their mutual innervations.
Intra-modal associative memory in the auditory cortex is also trained in the same manner. 
When associative information between visual and auditory data is provided, co-activation of associative memory cells induces mutual synapse innervations between associative memory cells, and thus, cross-modal associative memory cells are trained.
}
\label{fig:brain_associative_memory}
\end{figure}

==> tables/ablation.tex <==

\begin{table}[t]
\centering
\caption{The results of the ablation test for the training loss of the cross-modal association network. The ablation test is performed on the MNIST and GSC datasets.}
\label{tabular:ablation}
\begin{tabular}{c|c|cc}
%\begin{tabular}{|R|L|C{2cm}|C|C|C|C|C|}
\toprule
\multicolumn{1}{l}{} &\multicolumn{1}{l}{} &\multicolumn{2}{c}{Recognition Accuracy}        \\ \midrule
Dataset		&	Loss	&	Train (\%)	&	Test (\%)	\\ \midrule
\multirow{3}{*}{\shortstack{MNIST $\rightarrow$ GSC}}
&KLD	&	76.97	&	68.74	\\
&Recon.	&	9.98	&	10.32	\\
&KLD+Recon.	&	80.87	&	\textbf{75.02}	\\ \midrule
\multirow{3}{*}{\shortstack{GSC $\rightarrow$ MNIST}}
&KLD	&	92.15	&	\textbf{84.98}	\\
&Recon.	&	91.24	&	83.88	\\
&KLD+Recon.	&	92.75	&	84.47	\\
\bottomrule 
\end{tabular}
\end{table}

==> tables/comparison_rebuttal.tex <==

\begin{table}[t]%[bp]
% \centering
\footnotesize
\caption{Evaluation of cross-modal association models.}
%Accuracy is measured by the recognition model for the reconstructed data of the target modality from the input data of the other modality. Bold font denotes the best performance for each case.
\vspace{-0.5cm}
\begin{center}
\begin{tabular}{l|c|c|c|c}
\toprule
Model & GSC $\rightarrow$ 	& MNIST  & GSC $\rightarrow$  & GTSRB  \\
 &  MNIST	&  $\rightarrow$ GSC &  GTSRB &  $\rightarrow$ GSC \\
\midrule
baseline1               & 25.20  & 25.20  & 19.44  & 35.93 \\
baseline2               & 70.56  & 73.90  & 55.00  & 28.43 \\
JMVAE-zero $^{[3]}$     & 27.32  & 10.32  & 19.44  & 9.81 \\
JMVAE-kl$^{[3]}$        & 44.73  & 41.47  & 65.18  & 41.02 \\
CVA                     & 72.39  & 28.56  & 77.78  & 31.02 \\
MVAE$^{[4]}$            & 60.02  & 26.08  & 69.17  & 28.06 \\
\midrule
ours           & \textbf{84.47}  & \textbf{75.02}  & 75.09  & \textbf{59.63} \\
ours-all$^1$   & 83.18  & 73.80  & \textbf{77.87}  & 58.89 \\
ours-flex$^2$  & -      & -      & \textbf{80.56}  & \textbf{61.39} \\
\bottomrule 
\end{tabular}
%
% \begin{tabular}{l|c|c}
% \toprule
% Model & F-MNIST $\rightarrow$ GSC & F-MNIST $\rightarrow$ MNIST $\rightarrow$ GSC\\
% \midrule
% \textbf{ours} & 62.72 & 64.27\\                              
% \bottomrule 
% \end{tabular}
%
\end{center}
\vspace{-0.2cm}
$\qquad ^1$ add log-ratio term in (6)\\
$~\qquad ^2$ dim($z$) of GTSRB = 256 and dim($z$) of GSC = 64
\normalsize
\end{table}
% \vspace{-1.0cm}

